A MeerKAT view of the parsec-scale jets in the black-hole X-ray binary GRS 1758-258

Jets from accreting black hole (BH) X-ray binaries (XRBs) are powerful outflows that release a large fraction of the accretion energy to the surrounding environment, providing a feedback mechanism that may alter the interstellar medium (ISM) properties. Studying accretion and feedback together enables estimates of matter and energy input/output around accreting BHs. We focus on the extended jet structures of the BH-XRB GRS1758-258. First seen in VLA data, these parsec-scale jets arise from jet-ISM interaction and show a Z-shaped morphology. Using the MeerKAT telescope we observed GRS1758-258 in L-band for a total exposure of 7 hr. Applying a calorimetry-based method developed for AGN and later used for XRBs, we estimated the properties of the jets and of the surrounding ISM. We detect a jet and counter-jet terminating in bow-shocks. Within the northern jet lobe we identify synchrotron and bremsstrahlung emission, while the southern lobe is dominated by thermal emission. We measure ISM densities between 10-40 cm-3 across both jets, slightly lower in the northern region. The estimated ages of the two lobes range from 6-51 kyr. The time-averaged jet power lies between 4.4x10^33 and 3.3x10^36 erg/s, with differences between north and south likely due to different local ISM conditions. Comparing new MeerKAT with archival VLA data, we measured a proper motion of 130 mas/yr in a portion of the northern jet. Jet-ISM interaction structures on both sides of GRS1758-258 reveal different ISM properties. The comparison between these structures and those from other XRBs suggests that the lobes in GRS1758-258 are younger and may result from different jet activity phases. The time-averaged energy transferred to the environment is slightly lower than in other XRBs, consistent with the younger age of the lobes in GRS1758-258 relative to those of other systems.

==> def_bibtex.tex <==
\def\apj{ApJ}
\def\apjs{ApJ}
\def\mnras{MNRAS}
\def\aap{A\&A}
\def\apjl{ApJ}
\def\pasj{PASJ}
\def\nat{Nature}
\def\iaucirc{IAU Circ.}
\def\skytel{S\&T}
\def\aaps{A\&A S.S.}
\def\araa{Annual Reviews}
\def\apss{Ap\&SS}
\def\atel{The Astronomer's Telegram}
\def\jcap{Journal of Cosmology and Astroparticle Physics}
\def\ssr{Space Science Reviews}
\def\prd{Physical Review D}
\def\pasp{Publications of the Astronomical Society of the Pacific}
\def\na{New Astronomy}
